Delving into Transferable Adversarial Examples and Black-box Attacks

An intriguing property of deep neural networks is the existence of adversarial examples, which can transfer among different architectures. These transferable adversarial examples may severely hinder deep neural network-based applications. Previous works mostly study the transferability using small scale datasets. In this work, we are the first to conduct an extensive study of the transferability over large models and a large scale dataset, and we are also the first to study the transferability of targeted adversarial examples with their target labels. We study both non-targeted and targeted adversarial examples, and show that while transferable non-targeted adversarial examples are easy to find, targeted adversarial examples generated using existing approaches almost never transfer with their target labels. Therefore, we propose novel ensemble-based approaches to generating transferable adversarial examples. Using such approaches, we observe a large proportion of targeted adversarial examples that are able to transfer with their target labels for the first time. We also present some geometric studies to help understanding the transferable adversarial examples. Finally, we show that the adversarial examples generated using ensemble-based approaches can successfully attack Clarifai.com, which is a black-box image classification system.

==> ensemble-app.tex <==
\section{Further Results on Ensemble Attacks}
\label{app:ensemble}

In our experiments, we found that some models in the ensemble are easier to attack than
the others. To accommodate this in the optimization process, we can penalize the weights
of the models which have already been fooled. In particular, we keep $w_i^{(j)}$, where
$w_i^{(1)}=1$. At the beginning of iteration $j$ of the gradient descent, we set
$\alpha_i = \frac{w_i^{(j)}}{\sum_i w_i^{(j)}}$. After each iteration, we update $w_i^{(j+1)}$
as follows: if model $i$ can correctly predict the attack after the $j$-th iteration, then
$w_i^{(j+1)}\leftarrow w_i^{(j)}$; otherwise, $w_i^{(j+1)}\leftarrow \eta w_i^{(j)}$. Here,
$\eta$ is a decay constant. Also, in each iteration of the gradient descent,
we take the sign of the gradient as the update, instead of the gradient directly. Using
this approach, we can choose $\eta=0.9$ to get the results in Table~\ref{tab:alt-ensemble}

\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                  & RMSD  & \small ResNet-152 & \small ResNet-101 & \small ResNet-50 & \small VGG-16 & \small GoogLeNet \\ \hline
\small ResNet-152 & 17.05 & 4\%               & 0\%               & 0\%              & 0\%           & 0\%              \\ \hline
\small ResNet-101 & 16.89 & 1\%               & 3\%               & 0\%              & 0\%           & 1\%              \\ \hline
\small ResNet-50  & 17.08 & 1\%               & 1\%               & 2\%              & 0\%           & 1\%              \\ \hline
\small VGG-16     & 16.47 & 1\%               & 0\%               & 0\%              & 5\%           & 0\%              \\ \hline
\small GoogLeNet  & 16.32 & 0\%               & 0\%               & 0\%              & 0\%           & 5\%              \\ \hline
\end{tabular}
\caption{Row name means attack this model by ensemble of other models with multiplicative weight. Non-targeted attack with learning rate 5.0 terminates after 100 iterations.}
\label{tab:alt-ensemble}
\end{table}



==> exmp.tex <==
\section{Examples}

% Opt-based examples

\begin{figure}[t]
\begin{subfigure}[b]{0.32\textwidth}
\centering
  \includegraphics[scale=0.35]{image/ILSVRC2012_val_00049443/original-VGG16-crop.png}
  \caption{true label: anemone fish}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
  \includegraphics[scale=0.35]{image/ILSVRC2012_val_00049443/O-VGG16-4-T.png}
  \caption{targeted attack: file cabinet}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
  \includegraphics[scale=0.35]{image/ILSVRC2012_val_00049443/O-VGG16-4-NT.png}
  \caption{non-targeted attack}
\end{subfigure}
\end{figure}

% Clarifai results

\begin{figure}[t]
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00049443.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00042959.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00030794.png}
\end{subfigure}
\caption{Left column: original image. Middle column: attacks generated by Optimization method on ResNet-152. Right column: attacks generated by ensemble models(VGG16, GoogleNet, Inception, ResNet50, ResNet101, and ResNet152).}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00028723.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00010669.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00000475.png}
\end{subfigure}
\caption{Left column: original image. Middle column: attacks generated by Optimization method on ResNet-152. Right column: attacks generated by ensemble models(VGG16, GoogleNet, Inception, ResNet50, ResNet101, and ResNet152).}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00003062.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00005445.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00020946.png}
\end{subfigure}
\caption{Left column: original image. Middle column: attacks generated by Optimization method on ResNet-152. Right column: attacks generated by ensemble models(VGG16, GoogleNet, Inception, ResNet50, ResNet101, and ResNet152).}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00024304.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00027836.png}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.4]{image/Clarifai/00036060.png}
\end{subfigure}
\caption{Left column: original image. Middle column: attacks generated by Optimization method on ResNet-152. Right column: attacks generated by ensemble models(VGG16, GoogleNet, Inception, ResNet50, ResNet101, and ResNet152).}
\end{figure}


==> fast.tex <==
\section{Transferability Using Fast Gradient-based Approaches Using One Single Network}
\label{sec:transfer-fast}

We examine the fast gradient-based methods to generate the attacks.
These methods typically require computing the gradients only once, and thus
are much faster than optimization-based attacks. Such fast methods are popular,
since they can efficiently generate adversarial examples to facilitate the
retraining methods to improve models robustness.
%
In this work, we mainly examine two methods:
\paragraph{Fast gradient sign (FGS).} Proposed in~\cite{fast-gradient-sign}, fast
gradient sign can be used to generate adversarial images to meet the $L_\infty$
norm bound. The non-targeted adversarial examples are constructed as
\[x^\star \leftarrow \mathrm{clip}(x + B \mathbf{sgn}(\nabla_x \ell(J_\theta(x), \mathbf{1}_y)))\]
and the targeted ones are obtained by
\[x^\star \leftarrow \mathrm{clip}(x - B \mathbf{sgn}(\nabla_x \ell(J_\theta(x), \mathbf{1}_{y^\star})))\]
Here, $\mathrm{clip}(x)$ is used to clip each dimension of $x$ to $[0, 255]$.

\paragraph{Fast gradient (FG).} The term of $\mathbf{sgn}(\nabla_x \ell)$ 
is replaced by $\frac{\nabla_x \ell}{||\nabla_x \ell||})$,
where we assume $d(x, x^\star)=||x - x^\star||$, and $||\cdot||$ used in updates is the same
norm as used in the distance metric.

Here the coefficient $B$ is highly correlated with the RMSD. However RMSD typically has
a lower value than $B$, because of the clip operation and the zero elements in the gradients.
Therefore, we refer $B$ as the \emph{distortion} in the following discussion.

The fast-gradient approaches can be viewed as a coarse approximation to the solution of
optimization problem~(\ref{obj:non-targeted}) and~(\ref{obj:targeted}).
A good property of fast gradient-based approaches is that all adversarial examples lie in a
1-D subspace. Therefore, we can easily approximate the minimal distortion
of transferable adversarial examples between two models. In the rest of the section, we 
first study this approach to generate transferable adversarial images. Second, we control 
the RMSD, so that we can show results comparable to the optimization-based approaches
using one single model.


\newcommand{\effect}{adversarial images regression effect}

\subsection{Adversarial Images With Minimal Transferable Distortion}

For each image $x$, and two models $M_1, M_2$, we can determine the minimal
distortion $B$, such that $x_B=x+Bd$ generated for $M_1$ from $x^\star$ is 
adversarial for both $M_1$ and $M_2$. Here $d$ is the direction, i.e., 
$\mathbf{sgn}(\nabla_x\ell)$ for FGS and $\nabla_x\ell/||\nabla_x\ell||$ for FG.

We refer the RMSD between the transferable adversarial image $x_B$ and the 
original image $x$ as the \emph{minimal transferable RMSD} of $x$ from 
$M_1$ to $M_2$. We use minimal transferable RMSD to measure the tradeoff 
between distortion and transferability. We first show that
adversarial images may not occur in contiguous regions, and therefore,
we approximate for the minimal transferable distortion $B$ through a 
linear search. That is, we sample the value of $B$ every 0.1 step.

\paragraph{Adversarial images may not occur contiguous along the
adversarial direction.}
It is mentioned in~\cite{fast-gradient-sign} that along a direction $d$,
which aligns with $\mathbf{sgn}(\nabla_x \ell(J_\theta(x), \mathbf{1}_y))$, 
adversarial images occur contiguous. That is, there exists a threshold 
$B^\star$, such that $x_B=x+Bd$ is adversarial when $B\geq B^\star$, and benign 
if $B^\star>B\geq 0$. This was used to explain the existence of abundant adversarial 
images. Although, we agree on the latter conclusion, we observe the first 
statement may not always hold true. 
In Figure~\ref{fig:non-contiguous}, we show an example image, such that
its adversarial images on the gradient direction (i.e., $d=\nabla_x\ell$) of ResNet152
do not form one continuous interval, but they are segmented into three
regions (i.e., for $B\geq 0$).


\begin{figure}[t]
\begin{subfigure}{0.3\linewidth}
\centering
  \includegraphics[scale=0.5]{image/ILSVRC2012_val_00017691.png}
  \caption{The Image}
  \label{fig:linear-resnet}
\end{subfigure}
\begin{subfigure}{0.7\linewidth}
\centering
  \includegraphics[scale=0.5]{image/17691-VGG16-ResNet152-FG-NT.pdf}
  \caption{Prediction correctness}
  \label{fig:linear-vgg}
\end{subfigure}
\caption{The prediction correctness is computed as 1 if the adversarial image
is correctly predicted, and 0 otherwise. Here the adversarial noises are along
the non-targeted gradient direction for VGG16. $B$ is sampled every $0.1$ as a step.}
\label{fig:non-contiguous}
\end{figure}

\paragraph{Minimal transferable distortion.}

\begin{figure}[t]
\begin{subfigure}{0.5\linewidth}
\centering
  \includegraphics[scale=0.25]{image/FG-VGG16-ResNet152.png}
  \caption{Fast Gradient}
  \label{fig:tradeoff-fg}
\end{subfigure}
\begin{subfigure}{0.5\linewidth}
\centering
  \includegraphics[scale=0.25]{image/FGS-VGG16-ResNet152.png}
  \caption{Fast Gradient Sign}
  \label{fig:tradeoff-fgs}
\end{subfigure}
  \caption{The CDF of the minimal transferable RMSD 
  from VGG16 to ResNet152. The green line labels the median minimal transferable 
  RMSD, while the red line labels the minimal transferable RMSD to reach 90\% percentage.}
  \label{fig:tradeoff}
\end{figure}


Figure~\ref{fig:tradeoff} plots the cumulative distribution function (CDF) of the minimal
transferable RMSD from VGG16 to ResNet152 using non-targeted for fast gradient 
(Figure~\ref{fig:tradeoff-fg})
and fast gradient sign (Figure~\ref{fig:tradeoff-fgs}). From the figures, we observe that
both FGS and FG can find 100\% transferable adversarial images with large enough distortions.
Further, the fast gradient method can generate transferable attacks with smaller RMSD than
the fast gradient sign method. The reason is that while FGS minimizes the distortion's
$L_\infty$ norm, FG minimizes its $L_2$ norm, which is proportional to RMSD.
For targeted adversarial examples, most adversarial images cannot be predicted as the
targeted labels. So there is no meaningful result for targeted minimal transferable distortion.
We will discuss this issue more in the next subsection.


\subsection{Comparison With Optimization-based Methods}

In Table~\ref{tab:trans-fg}, we choose $B$ such that the average RMSD of the adversarial images generated using the
fast-gradient approach is almost the same as those generated using the 
optimization-based approach (Table~\ref{tab:non-targeted-opt}).
We observe that the diagonal of the Table~\ref{tab:trans-fg} is higher than Table~\ref{tab:non-targeted-opt}, which means
that the fast-gradient approach is not as effective as the optimization-based approaches to generate adversarial examples
for one model to attack itself. This is reasonable because the fast-gradient approach can be viewed as a way
to approximate the optimization, but tailored for speed over accuracy.

On the other hand, the accuracy of adversarial images generated for one model 
but evaluated on another, however, is generally lower than their counterparts 
in the optimization-based approach. A potential reason is as follows. Consider 
for any model, there exists an high-dimensional subspace composed by all 
adversarial examples. We call this \emph{the adversarial subspace} of the 
model. While non-targeted optimization-based approach optimizes~
(\ref{obj:non-targeted}), the algorithm searches the entire adversarial 
subspace of one model, which is more likely to be out of the adversarial 
subspace of the other model. For the fast gradient approach, the algorithm 
only searches the 1-D projection of the adversarial subspace, whose 
overlapping with the counterpart of the other model is larger.\chang{Need to think about this more.}
Therefore it is more likely to find common adversarial examples for both models,
which are transferable adversarial examples. For this reason, we intuitively 
say the adversarial examples generated using optimization-based approach ``overfitting"
to the model using during generation.

We also evaluate the fast gradient sign method, but its transferability is 
worse than both fast gradient and optimization-based approaches. However, 
we find that when configuring the average RMSD to be around 23, the distortion 
is not as high as the counterparts for optimization-based approach and FG. 
We intuitively say that these adversarial images generated using FGS is 
``underfitting" to the model using during generation. 
We present the results in Appendix~\ref{app:fg} (Table~\ref{tab:trans-fgs}).

\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                  & RMSD  & \small ResNet152 & \small ResNet101 & \small ResNet50 & \small VGG16 & \small GoogLeNet & \small Incept-v3 \\ \hline
\small ResNet152 & 23.45 & 4\%               & 13\%              & 13\%             & 20\%          & 12\%             & 31\%             \\ \hline
\small ResNet101 & 23.49 & 19\%              & 4\%               & 11\%             & 23\%          & 13\%             & 36\%             \\ \hline
\small ResNet50  & 23.49 & 25\%              & 19\%              & 5\%              & 25\%          & 14\%             & 36\%             \\ \hline
\small VGG16     & 23.73 & 20\%              & 16\%              & 15\%             & 1\%           & 7\%              & 15\%             \\ \hline
\small GoogLeNet  & 23.45 & 25\%              & 25\%              & 17\%             & 19\%          & 1\%              & 29\%             \\ \hline
\small Incept-v3  & 23.35 & 45\%              & 48\%              & 29\%             & 31\%          & 27\%             & 22\%             \\ \hline
\end{tabular}
\caption{Transferability between pairs of models using fast gradient method. The first column means the average RMSD of all
adversarial images generated for the model in the corresponding row. The cell $(i, j)$ indicates the accuracy of the
adversarial images generated for model $i$ (row) evaluated over model $j$ (column). Lower accuracy indicates better transferability.}
\label{tab:trans-fg}
\end{table}

\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
                  & \small ResNet-152 & \small ResNet-101 & \small ResNet-50 & \small VGG-16 & \small GoogLeNet & \small Inception \\ \hline
\small ResNet-152 & 100.00\%          & 33.33\%           & 24.00\%          & 17.50\%       & 15.38\%          & 18.06\%          \\ \hline
\small ResNet-101 & 33.33\%           & 100.00\%          & 35.00\%          & 19.05\%       & 14.81\%          & 21.05\%          \\ \hline
\small ResNet-50  & 24.00\%           & 35.00\%           & 100.00\%         & 21.18\%       & 13.10\%          & 21.79\%          \\ \hline
\small VGG-16     & 17.50\%           & 19.05\%           & 21.18\%          & 100.00\%      & 15.05\%          & 18.82\%          \\ \hline
\small GoogLeNet  & 15.38\%           & 14.81\%           & 13.10\%          & 15.05\%       & 100.00\%         & 17.07\%          \\ \hline
\small Inception  & 18.06\%           & 21.05\%           & 21.79\%          & 18.82\%       & 17.07\%          & 100.00\%         \\ \hline
\end{tabular}
\caption{When we using fast gradient approach for VGG16 model, 
cell $(i, j)$ is the percentage of all adversarial images that 
are prediected as the same wrong labels by both models $i$ and $j$.}
\end{table}

\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
           & RMSD  & ResNet-152 & ResNet-101 & ResNet-50 & VGG-16 & GoogLeNet & Inception \\ \hline
ResNet-152 & 23.11 & 12\%       & 27\%       & 25\%      & 22\%   & 15\%      & 51\%      \\ \hline
ResNet-101 & 23.11 & 29\%       & 13\%       & 29\%      & 29\%   & 16\%      & 55\%      \\ \hline
ResNet-50  & 23.11 & 34\%       & 28\%       & 10\%      & 25\%   & 23\%      & 46\%      \\ \hline
VGG-16     & 23.12 & 25\%       & 20\%       & 23\%      & 0\%    & 8\%       & 22\%      \\ \hline
GoogLeNet  & 23.11 & 46\%       & 41\%       & 40\%      & 25\%   & 2\%       & 49\%      \\ \hline
Inception  & 23.03 & 62\%       & 62\%       & 51\%      & 45\%   & 36\%      & 35\%      \\ \hline
\end{tabular}
\caption{Transferability between pairs of models using fast gradient sign method. The first column means the average RMSD of all
adversarial images generated for the model in the corresponding row. The cell $(i, j)$ indicates the accuracy of the
adversarial images generated for model $i$ (row) evaluated over model $j$ (column). Lower accuracy indicates better transferability.}
\end{table}

\begin{table}[t]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
                  & \small ResNet-152 & \small ResNet-101 & \small ResNet-50 & \small VGG-16 & \small GoogLeNet & \small Inception \\ \hline
\small ResNet-152 & 100.00\%          & 33.78\%           & 36.62\%          & 16.00\%       & 14.86\%          & 20.59\%          \\ \hline
\small ResNet-101 & 33.78\%           & 100.00\%          & 43.24\%          & 20.00\%       & 20.25\%          & 21.13\%          \\ \hline
\small ResNet-50  & 36.62\%           & 43.24\%           & 100.00\%         & 23.38\%       & 13.16\%          & 22.06\%          \\ \hline
\small VGG-16     & 16.00\%           & 20.00\%           & 23.38\%          & 100.00\%      & 19.57\%          & 23.08\%          \\ \hline
\small GoogLeNet  & 14.86\%           & 20.25\%           & 13.16\%          & 19.57\%       & 100.00\%         & 16.22\%          \\ \hline
\small Inception  & 20.59\%           & 21.13\%           & 22.06\%          & 23.08\%       & 16.22\%          & 100.00\%         \\ \hline
\end{tabular}
\caption{When we using fast gradient sign approach for VGG16 model, 
cell $(i, j)$ is the percentage of all adversarial images that 
are prediected as the same wrong labels by both models $i$ and $j$.}
\end{table}


We also evaluated targeted adversarial examples. 

We also evaluated targeted adversarial examples. 
However, we also observe that the labels do not transfer. The results are
deferred to Appendix~\ref{app:fg} Table~\ref{tab:fg-targeted}.
Different from optimization-based approaches, however, most targeted attacks do not
mislead the model used to generate the attack to predict the targeted labels.
We attribute it to the fact that fast-gradient-based approaches only search for attacks
in a 1-D subspace, in which the possible predictions
may constitute a small subset of all labels. In this case, for most of the targeted
labels, it is impossible for the generated attacks meet the targeted labels.


==> trans.tex <==
\section{Transferability of Optimization-based Approaches Using One Single Network}
\label{sec:transfer}

We first examine the transferability if we generate adversarial
images by optimizing~(\ref{obj:non-targeted}) and (\ref{obj:targeted})
directly. We use Adam Optimizer~\cite{adam}, initialize $x^\star$ to be
$x$. We find that we can tune the RMSD by tuning the learning rate of
Adam and $\lambda$. When we set the learning rate to be small, and
choose whatever $\lambda$ (i.e., which may even be 0), it is easy
to generate adversarial images for each model with small RMSD, i.e. $<2$. 
However, these adversarial images cannot transfer well to other models
(see Appendix~\ref{app:opt} for details).

Therefore, we increase the learning rate and set $\lambda=0$ to allow
the optimization algorithm to search for adversarial images with larger
distortion. Notice that an alternative method to achieve this goal is
revise the optimization objective to incorporate this RMSD constraint.
For example, for non-targeted adversarial image searching, we can optimize
for the following objective.
\[\mathbf{argmin}_{x^\star} -\log{(1-J_\theta(x^\star)_y)} + \lambda_1 \mathrm{ReLU}(\tau - d(x, x^\star)) + \lambda_2 \mathrm{ReLU}(d(x, x^\star) - \tau)\]
Optimizing for the above objective has the following three effects: 
(1) minimizing $-\log{(1-J_\theta(x^\star)_y)}$;
(2) Penalizing the solution if $d(x, x^\star)$ is no more than a threshold $\tau$ (too low); and
(3) Penalizing the solution if $d(x, x^\star)$ is too high.

In our evaluation, however, we found that the solutions computed from
the two approaches have equivalent transferability. Therefore, in this work, 
we take the first approach. In particular, we set learning rate to be $4$. 
We run Adam Optimizer for 100 iterations to generate the adversarial images, 
when the loss converges. 

\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                  & RMSD  & \small ResNet152 & \small ResNet101 & \small ResNet50 & \small VGG16 & \small GoogLeNet & \small Incept-v3 \\ \hline
\small ResNet152 & 22.83 & 0\%               & 13\%              & 18\%             & 19\%          & 11\%             & 44\%             \\ \hline
\small ResNet101 & 23.81 & 19\%              & 0\%               & 21\%             & 21\%          & 12\%             & 45\%             \\ \hline
\small ResNet50  & 22.86 & 23\%              & 20\%              & 0\%              & 21\%          & 18\%             & 37\%             \\ \hline
\small VGG16     & 22.51 & 22\%              & 17\%              & 17\%             & 0\%           & 5\%              & 16\%             \\ \hline
\small GoogLeNet  & 22.58 & 39\%              & 38\%              & 34\%             & 19\%          & 0\%              & 49\%             \\ \hline
\small Incept-v3  & 23.02 & 56\%              & 50\%              & 44\%             & 35\%          & 27\%             & 0\%              \\ \hline
\end{tabular}
\caption{Transferability of non-targeted adversarial images between pairs of models. The first column means the average RMSD of all
adversarial images generated for the model in the corresponding row. The cell $(i, j)$ indicates the accuracy of the
adversarial images generated for model $i$ (row) evaluated over model $j$ (column). Lower accuracy indicates better transferability.}
\label{tab:non-targeted-opt}
\end{table}

The results are presented in Table~\ref{tab:non-targeted-opt}.
From the tables, we can observe that
\begin{itemize}
\item The diagonal contains all 0 values. This says that all 
    adversarial images generated for one model can totally fool this model.
\item VGG16 is more effective to be used to generate transferable attacks
    than other models. For example, although the three ResNet models share
    similar architectures which differ only in the hyperparameters,
    VGG16's adversarial images have lower accuracy on ResNet152 than both
    ResNet50 and ResNet101. %\chang{We do not understand the reason.}
\item The intuition that a more performant model can be used to generate
    more transferable attacks is wrong. We observe that VGG16, which can only
    outperform GoogLeNet, can generate the most transferable attacks, while the
    state-of-the-art model, Inception-v3,
    generates the least transferable attacks.
\end{itemize}


\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
           & \small RMSD & \small ResNet152 & \small ResNet101 & \small ResNet50 & \small VGG16 & \small GoogLeNet & \small Incept-v3 \\ \hline
\small ResNet152 & 23.13 & 100\%      & 2\%        & 1\%       & 1\%    & 1\%       & 0\%       \\ \hline
\small ResNet101 & 23.16 & 3\%        & 100\%      & 3\%       & 2\%    & 1\%       & 1\%       \\ \hline
\small ResNet50  & 23.06 & 4\%        & 2\%        & 100\%     & 1\%    & 1\%       & 0\%       \\ \hline
\small VGG16     & 23.59 & 2\%        & 1\%        & 2\%       & 100\%  & 1\%       & 0\%       \\ \hline
\small GoogLeNet  & 22.87 & 1\%        & 1\%        & 0\%       & 1\%    & 100\%     & 0\%       \\ \hline
\small Incept-v3  & 22.74 & 0\%        & 0\%        & 0\%       & 0\%    & 0\%       & 100\%     \\ \hline
\end{tabular}
\caption{Cell $(i, j)$ indicates that percentage of the targeted adversarial images
 generated for model $i$ (row)
is predicted as the targeted label by model $j$ (column). Higher value indicates more successful
transferable targeted labels.}
\label{tab:matching-target-opt}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                  & RMSD  & \small ResNet-152 & \small ResNet-101 & \small ResNet-50 & \small VGG-16 & \small GoogLeNet & \small Inception \\ \hline
\small ResNet-152 & 31.35 & 98\%              & 1\%               & 2\%              & 2\%           & 0\%              & 0\%              \\ \hline
\small ResNet-101 & 31.11 & 5\%               & 98\%              & 1\%              & 2\%           & 0\%              & 0\%              \\ \hline
\small ResNet-50  & 31.32 & 3\%               & 2\%               & 99\%             & 1\%           & 1\%              & 1\%              \\ \hline
\small VGG-16     & 31.50 & 1\%               & 1\%               & 2\%              & 97\%          & 1\%              & 0\%              \\ \hline
\small GoogLeNet  & 30.67 & 2\%               & 1\%               & 0\%              & 2\%           & 97\%             & 0\%              \\ \hline
\small Inception  & 33.27 & 0\%               & 0\%               & 0\%              & 0\%           & 0\%              & 100\%            \\ \hline
\end{tabular}
\caption{Cell $(i, j)$ indicates that percentage of the targeted adversarial images
 generated for model $i$ (row)
is predicted as the targeted label by model $j$ (column). Higher value indicates more successful
transferable targeted labels. We used higher learning rate to achieve larger RMSD.}
\label{tab:matching-target-opt}
\end{table}


Table~\ref{tab:matching-target-opt} presents the results for targeted adversarial examples. 
We observe that (1) the targeted adversarial images' prediction can match
the targeted labels when evaluated on the same model that is used to generated the adversarial examples; 
but (2) the targeted adversarial images cannot be rarely predicted as the targeted labels 
by a different model. We call the later that \emph{the targeted labels do not transfer}. As we will 
see later, when generating targeted adversarial images using one single model, we do not observe
the targeted labels transfer.

%\begin{table}[t]
%\centering
%\begin{tabular}{c}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%                  & \small ResNet152 & \small ResNet101 & \small ResNet50 & \small VGG16 & \small GoogLeNet & \small Incept-v3 \\ \hline
%\small ResNet152 & 100.00\%            & 28.57\%             & 29.87\%            & 19.23\%         & 12.82\%            & 17.81\%            \\ \hline
%\small ResNet101 & 28.57\%             & 100.00\%            & 40.00\%            & 18.07\%         & 20.48\%            & 23.38\%            \\ \hline
%\small ResNet50  & 29.87\%             & 40.00\%             & 100.00\%           & 22.89\%         & 18.07\%            & 21.05\%            \\ \hline
%\small VGG16     & 19.23\%             & 18.07\%             & 22.89\%            & 100.00\%        & 16.84\%            & 25.00\%            \\ \hline
%\small GoogLeNet  & 12.82\%             & 20.48\%             & 18.07\%            & 16.84\%         & 100.00\%           & 17.28\%            \\ \hline
%\small Incept-v3  & 17.81\%             & 23.38\%             & 21.05\%            & 25.00\%         & 17.28\%            & 100.00\%           \\ \hline
%\end{tabular}
%\end{tabular}
%\caption{When using optimization-based approach for VGG16 model,
%cell $(i, j)$ is the percentage of all adversarial images that are predicted as the same labels
%by both models $i$ and $j$.}
%\end{table}
%
%\paragraph{Non-targeted labels.}

%\begin{table}[t]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\multicolumn{2}{|c|}{ResNet-152}        & \multicolumn{2}{c|}{ResNet-101}        & \multicolumn{2}{c|}{ResNet-50} \\ \hline
%52.6\%         & apron                & 100.0\%        & window screen       & 90.5\%   & tennis ball       \\ \hline
%24.9\%         & brain coral          & \multicolumn{2}{c|}{\multirow{4}{*}{}} & 7.8\%    & chainlink fence   \\ \cline{1-2} \cline{5-6}
%22.5\%         & chain mail           & \multicolumn{2}{c|}{}                  & 0.9\%    & coral reef        \\ \cline{1-2} \cline{5-6}
%0.1\%          & stingray             & \multicolumn{2}{c|}{}                  & 0.6\%    & brain coral       \\ \cline{1-2} \cline{5-6}
%\multicolumn{2}{|c|}{}                  & \multicolumn{2}{c|}{}                  & 0.1\%    & chain             \\ \hline
%\multicolumn{2}{|c|}{VGG-16}            & \multicolumn{2}{c|}{GoogLeNet}         & \multicolumn{2}{c|}{Inception} \\ \hline
%100.0\%        & boa constrictor      & 87.2\%         & window screen       & 37.4\%   & binder            \\ \hline
%\multicolumn{2}{|c|}{\multirow{4}{*}{}} & 10.2\%         & velvet              & 32.6\%   & jellyfish         \\ \cline{3-6}
%\multicolumn{2}{|c|}{}                  & 2.2\%          & prayer rug          & 13.8\%   & velvet            \\ \cline{3-6}
%\multicolumn{2}{|c|}{}                  & 0.1\%          & jigsaw puzzle       & 10.3\%   & necklace          \\ \cline{3-6}
%\multicolumn{2}{|c|}{}                  & 0.1\%          & envelope            & 5.0\%    & wool              \\ \hline
%\end{tabular}
%\caption{Top 5 most frequently predicted labels on random images. We sample 100,000 random images, i.e., every pixel value is uniformly
%randomly chosen from $[0, 255]$, and compute the prediction of random images to compute the frequency of labels for each model.}
%\end{table}

==> transform.tex <==
\section{Transformation Effects on Transferability}
\label{sec:transform}

